Dynamic Mini-batch SGD for Elastic Distributed Training: Learning in the Limbo of Resources

With an increasing demand for training powers for deep learning algorithms and the rapid growth of computation resources in data centers, it is desirable to dynamically schedule different distributed deep learning tasks to maximize resource utilization and reduce cost. In this process, different tasks may receive varying numbers of machines at different time, a setting we call elastic distributed training. Despite the recent successes in large mini-batch distributed training, these methods are rarely tested in elastic distributed training environments and suffer degraded performance in our experiments, when we adjust the learning rate linearly immediately with respect to the batch size. One difficulty we observe is that the noise in the stochastic momentum estimation is accumulated over time and will have delayed effects when the batch size changes. We therefore propose to smoothly adjust the learning rate over time to alleviate the influence of the noisy momentum estimation. Our experiments on image classification, object detection and semantic segmentation have demonstrated that our proposed Dynamic SGD method achieves stabilized performance when varying the number of GPUs from 8 to 128. We also provide theoretical understanding on the optimality of linear learning rate scheduling and the effects of stochastic momentum.

==> old_evaluation.tex <==
%auto-ignore

%\section{Evaluation}
\section{Experimental Results} \label{experiment}

In this section, we first study the behavior of two basic strategies with no tailing nor square root scaling rule when there is a sudden change of available GPUs and per-GPU batch size on the ImageNet~\cite{deng2009imagenet} dataset.
We also explore the limitation of fixing total batch size training and fixing per-GPU batch size training and benchmark the improvement using stable tailing and square-root learning-rate scaling strategies. 
Then we evaluate the robustness of proposed methods with different random GPU schedules. 
Finally, we apply elastic distributed training on object detection using Single Shot Multi-box Object Detector (SSD)~\cite{liu2016ssd}.


% We compare baseline models trained with a fixed number of workers, and models trained with dynamic number of workers in this approach under 5 different worker schedules for simulation. For each method, we start with perturbing the training process by adding or removing workers at specific epochs to study their impact to optimization. Then we extend our experiment with randomly generated schedules to simulate multiple changes. We discuss detailed experimental results on image classification on the ImageNet dataset, and then also share results of the object detection task with single shot multi-box detector on the MS COCO dataset\cite{russakovsky2015imagenet, lin2014microsoft}.

\subsection{Baseline Methods}


\paragraph{Fixed Total Batch Size}
\label{sec:fix_total}

In this strategy, the total batch size is fixed through the whole training process. 
The per-worker batch size is dynamically calculated based on the number of available workers.
In the case that the total batch size cannot be divided evenly, a subset of workers are assigned with 1 more samples than others. 
This strategy does not change how a single batch is computed compared to normal data parallel distributed SGD illustrated in Algorithm~\ref{algo:data_para}, except that the number of workers $N$ and per-worker batch size $S$ may change from batch to batch. 


This strategy may not affect the optimization process and results in the same model 
convergence despite the change of number of workers, if the model does not %contain modules different 
change its behaviors according to the per-worker batch size. %, e.g. batch normalization. 
%But when
However, Batch Normalization has become de facto standard in modern CNN architectures, which introduces extra difficulty for fixed total batch size method. %we may have constraints on the maximal number of workers. 
Previous studies~\cite{wu2018group, Zhang_2018_CVPR} show that a too small per-worker batch may cause degraded final model quality, but they are not directly applicable in our work as discussed in Section~\ref{sec:related}.
% Instead, we propose a simple but effective strategy to increase the per-work batch size 
% in the last few training epochs, so that the network can optimize the batch statistics
% in the Batch Normalization layers. 
% This strategy is easy to achieve, as we can always choose not to use extra workers. 
% We refer to the approach of enlarging the per-worker batch size near the end of the training process as {\it Stable Tailing} strategy.



%\paragraph{Baseline Models}
\paragraph{Implementation Details}
% Baseline models, dataset, Hyper-parameters: lr, wd, Other Strategies: lr scaling
We adapt ResNet50~\cite{he2016deep} as the baseline model and evaluate the performance on ImageNet2012~\cite{deng2009imagenet} dataset. The network is trained for 90 total number of epochs using a cosine learning rate scheduling~\cite{DBLP:journals/corr/LoshchilovH16a}.
The learning rate is warmed-up for 5 epochs~\cite{goyal2017accurate}. We use stochastic gradient descent (SGD) optimizer and set the momentum as 0.9 and weight decay as 0.0001. We use 8 GPUs with 128 per-GPU batch size as the baseline and set the base learning rate as 0.4. We linearly scale up the learning rate when increasing the global batch size.
%We use baseline$_{S}$ to denote a baseline model trained with a per-worker batch size of $S$ using a fixed number of workers. We use ResNet-50 v1b, trained on the ISLVRC2012~\cite{deng2009imagenet} dataset. 
%The model is trained with 5 epochs to warm up the learning rate linearly from zero to the original starting value~\cite{goyal2017accurate}, then decayed overtime using the cosine learning rate schedule \cite{DBLP:journals/corr/LoshchilovH16a} until epoch 90. Following Goyal, Priya, et al~\cite{DBLP:journals/corr/GoyalDGNWKTJH17} we also initialize the gamma parameter of the last batch normalization layer of each ResNet block to zero. We initialize all bias vectors of convolutional and fully-connected layers to zero following common practice. Xavier algorithm is used to initialize the weight matrices of convolutional and fully-connected layers~\cite{glorot2010understanding}.


\subsection{Basic Strategies}

We first conduct a study on the impact of a sudden increase of available GPUs during the training. The top-1 accuracy on the ImageNet~\cite{deng2009imagenet} validation set is used in this evaluation.
%using standard fix total batch size training and fix worker batch size training strategies.


\begin{table}
\centering
\begin{adjustbox}{max width=\linewidth}

\begin{tabular}{|l|l|l|l|l|}
  \hline
  Strategy & \# GPUs & BS    & LR & Top-1 Acc           \\ \hline
  Baseline & 8         & 128   & 1x  & 76.89\%             \\ \hdashline
  Fixed total, w/o tailing & 64        & 16 & 1x      & 76.37\% ($-$0.52\%) \\
  %12        &     & 76.28\% ($-$0.61\%) \\
  Fixed total, w/o tailing & 128      & 8   & 1x    & 75.04\% ($-$1.85\%) \\ \hdashline
  Fixed worker, linear & 64       & 128  & 8x     & 76.18\% ($-$0.71\%) \\
  %12        &     & 74.49\% ($-$2.40\%) \\
  Fixed worker, linear & 128        & 128 & 16x     & 76.09\% ($-$0.80\%) \\
  \hline
  \end{tabular}

\end{adjustbox}

  \caption{The influences of the number of GPUs and per-GPU batch size when basic strategies are in use. Top-1 validation accuracy on ImageNet dataset using single-crop. The number of GPUs increases at epoch 20. ({\it BS} denotes per-GPU batch size.)
  %The total batch size for all experiments is 1024. Baseline$_{128}$ is trained with a per-worker batch size of 128, using 8 workers. Experiments with spike schedule start with 8 workers, and increase the number of workers to 64, 96, and 128 respectively at epoch 20. Baseline$_{128}$ is trained with a extremely small per-worker batch size of 8 using 128 workers.
  }
  \label{tab:ablation}
\end{table}

We consider two simple strategies:
1) fixing the global batch size, and set per-worker batch size according to available nodes.
2) fixing per-worker batch size. The baseline model achieves 76.89\% top-1 accuracy on the validation set.
We observe that the accuracy drops for both strategies, when the number of available GPUs is increased.
Table~\ref{tab:ablation} shows that training with more GPUs are more difficult to optimize either due to increased total batch size or reduced per-GPU batch size.
Notice that the fixed total batch size strategy leads to small per-worker batch sizes.
This results in inaccurate batch statistics and suffers up to 1.85\% loss of accuracy.
Meanwhile the fixed worker strategy loses up to 0.80\% of accuracy due to a sudden change in learning rate. 

% We denote a ResNet-50 base model trained with learning rate $\hat \alpha$, total batch size $\hat B$ and $\hat K$ workers, as $base_{\hat B, \hat K}$. For instance, $base_{1024,8}$ refers to a ResNet-50 model trained with total batch size 1024 and 8 workers, each worker assigned with a batch of 128 samples per iteration.

% Two base models are trained with a fixed total batch size of 1024, with per-worker batch size $S$ set to 128 and 8, reaching 76.89\% and 74.76\% Top-1 validation accuracy respectively. As expected, with $S$ = 8 the model performs much worse due to the small mini-batch size used for BN.

% : $base_{1024, 128}$ and $base_{1024, 8}$, which use a fixed total size of 1024, with 128 and 8 GPUs respectively. $base_{1024, 8}$ uses a per worker mini-batch size of 128 and reaches 76.89\% validation accuracy, while $base_{1024, 128}$ performs 2.13\% worse than $base_{1024, 8}$, due to a very small mini-batch size per worker (8 images) for batch normalization.



\begin{comment}

% You may not need to explicitly mention them in a section, probably separate them into different sections
\subsection{Scheduling}

%\subsubsection{Worker Schedules}

For simplicity, we assume that the number of workers does not change in the middle of any epoch, and $K_e$ denotes the number of workers at epoch $e$. We also assume that the number of workers does not change during the first 5 epochs. $r$ denotes the scale of which the number of workers changes to. The visualization of these worker schedules are shown in Figure~\ref{fig:sched_viz}.

\begin{enumerate}
\item \fixed{}: $K_t$ is fixed all the time. All base models are trained with this schedule.

\item $spike(e, r)$: $K_t$ remains $\hat K$ for the first $e$ epochs and changes to $r\hat K$ thereafter.

\item $damp(e, r)$: $K_t$ remains $\hat K$ for the first $e$ epochs and changes to $\hat K/r$ thereafter.

% \begin{equation}
%   K_t=\left\{
%   \begin{array}{@{}ll@{}}
%     \hat K, & \text{if}\ t < e \\
%     r\hat K, & \text{otherwise}
%   \end{array}\right.
% \end{equation}

% \item $reg\_switch(e, r)$: $K_t$ regularly switches between $\hat K$ and $r\hat K$ every $e$ epochs.

% \begin{equation}
%   K_t=\left\{
%   \begin{array}{@{}ll@{}}
%     \hat K, & \text{if}\ t \mod 2e < e \\
%     r\hat K, & \text{otherwise}
%   \end{array}\right.
% \end{equation}

\item $rand\_switch(p, r)$: $K_t$ switches between $\hat K$ and $r\hat K$ with probability $p$ at each epoch.

\item $rand\_step(e, r)$: $K_t$ is a random integer between $\hat K$ and $r\hat K$ every $e$ epochs.

% \begin{equation}
%   K_t=\left\{
%   \begin{array}{@{}ll@{}}
%     \hat K, & \text{if} \ t = 0 \\
%     r{\hat K}^2 / K_{t-1}, & \text{if}\ rand() < p, t > 0 \\
%     K_{t-1}, & \text{otherwise}
%   \end{array}\right.
% \end{equation}

% \begin{equation}
%   K_t= (randint(r) + 1) * \hat K
% \end{equation}

\end{enumerate}


\begin{figure*}[tp]
\centering
\subfigure[fixed]{
\includegraphics[width=.17\textwidth]{plot/sched_fixed.pdf}
}
\subfigure[spike(20, 4)]{
\includegraphics[width=.17\textwidth]{plot/sched_spike.pdf}
}
\subfigure[damp(20, 4)]{
\includegraphics[width=.17\textwidth]{plot/sched_damp.pdf}
}
\subfigure[rand\_switch(0.5, 4)]{
\includegraphics[width=.17\textwidth]{plot/sched_rand_switch.pdf}
}
\subfigure[rand\_step(5, 4)]{
\includegraphics[width=.17\textwidth]{plot/sched_rand_step.pdf}
}
\caption{Visualization of 5 worker schedules.}
\label{fig:sched_viz}
\end{figure*}



\end{comment}



\subsection{Fixing Total Batch Size with Stable Tailing}

For fixing total batch size, we dynamically scale down the per-GPU batch size. As discussed in Section~\ref{sec:fix_total}, the batch normalization only considers the per-GPU batch statistics, and the performance of a network may drop with limited per-GPU batch size. We hypothesize that the performance of fixing total batch size training is impaired by the degraded batch statistics. 
We first visualize the batch statistics of batch normalization layers in the network in Figure~\ref{fig:bn_viz_big}. We find the batch variances have very different distributions for the per-GPU batch size of 8 and 128. 
For this, we adapt the stable tailing strategy which decreases the number of GPUs to 8 in the last 5 epochs resulting in a per-GPU batch size of 128, so that the batch statistics can be updated. 
For comparison, we evaluate the models training with constant per-GPU batch size of 8 or 128 (denoted as  {\it Baseline$_8$ and Baseline$_{128}$}) and increasing the number of GPUs at the last 5 epochs as the baseline approaches. The validation accuracy curves are shown in Figure~\ref{fig:fixed_adapt}. 
We find that the per-GPU batch size of the last 5 epochs will dramatically affect the network accuracy. 
We further evaluate the effect of stable tailing strategy using different number of GPUs in Table~\ref{tab:tailing_comp}, and find the performance is often improved using stable tailing strategy.

% \paragraph{Scale Evaluations}
% \label{sec:scale_eval_fixed_total}

% Since DPBS dynamically scales the per-worker batch size, a large number of workers results in a small batch size per worker. As pointed out previously, batch normalization relies on per-worker batch statistics, and may break down if the batch is too small.

% In Table~\ref{tab:scale_fixed_bs}, the number of workers spikes at epoch 20 to different scales. Both baseline$_{128}$ and baseline$_{8}$ are trained with a total batch size of 1024. Baseline$_{128}$ uses a per-worker batch size of 128, and 8 workers. Baseline$_{128}$, in contrast, uses a extremely small per-worker batch size of 8, and 128 workers. Such a small per-worker batch size leads to 2.13\% worse in validation accuracy compared to that of baseline$_{128}$. All DPBS experiments uses the same total batch size of 1024 and start with 8 workers. At epoch 20, the number of workers increases to 64, 96, and 128 respectively, and remains for the rest of 70 epochs. The greater the scale, the worse accuracy.




% \paragraph{Adaptability Evaluations}

% The previous paragraph shows that performance worsens if a sub-optimal per-worker batch size (e.g. 8 samples per worker) is used for a long time. Given a model trained with such a sub-optimal per-worker batch size for a long time, is it possible to fix the performance if the last few epochs are trained with a sufficient batch size?

% To answer this question, we run the following experiment, as shown
% in in Figure~\ref{fig:fixed_adapt}(a). All four experiments are
% trained with a total batch size of 1024. Baseline$_{128}$ uses a
% per-worker batch size of 128, and 8 workers. Baseline$_{128}$ uses
% a extremely small per-worker batch size of 8, and 128 workers.
% The spike schedule starts with 8 workers for the first 80 epochs (same as baseline$_{128}$), and boosts the number of workers to 128 at epoch 80. Conversely, the damp schedule uses with 128 workers for the first 80 epochs (same as baseline$_{8}$), and reduces the number of workers to 8 for the last 10 epochs. Comparing spike schedule and the baseline$_{8}$, one epoch of sub-optimal per-worker batch size causes performance degradation and the training trajectory merges within a few epochs. Comparing damp schedule and the baseline$_{128}$, one epoch of proper per-worker batch size (128 samples per worker) increases the validation accuracy as much as 1.86\%.
% Such property provides a ``safety net'' that even if the network is trained with sub-optimal per-worker batch size for a long time, we can mitigate the accuracy loss by switching to a normal per-worker batch size at the final epochs of the training.
% The visualization result in Figure ~\ref{fig:bn_viz_big} suggests that switching to a normal batch size for BN helps stablize the BN parameters during training.


\begin{figure*}[t!]
\centering
%\subfigure[baseline$_{128}$, epoch 84]{
%\includegraphics[width=.2\textwidth]{plot/bn/bn_base_84.png}
%}
%\subfigure[baseline$_{128}$, epoch 89]{
%\includegraphics[width=.2\textwidth]{plot/bn/bn_base_89.png}
%}
\subfigure[BS=8, epoch 84]{
\includegraphics[width=.2\textwidth]{plot/bn/bn_damp_84.png}
}
\subfigure[BS=128, epoch 84]{
\includegraphics[width=.2\textwidth]{plot/bn/bs_128_epoch=84_step_schedule.png}
}
\subfigure[BS=8 tailing, epoch 89]{
\includegraphics[width=.2\textwidth]{plot/bn/bn_damp_89.png}
}
\subfigure[BS=128, epoch 89]{
\includegraphics[width=.2\textwidth]{plot/bn/bs=128_epoch=89_step_schedule}
}
\caption{
Visualization of Batch Norm parameters distributions. Showing histogram of the running variances of batch normalization layer at stage 2, block 0. 
%The histograms shows the data distribution over optimization steps (4540 ... 6000). 
%Figure (a) and (b) are the visualization for the baseline$_{128}$ at epoch 84 and 89. The baseline model is trained with step-wise learning rate schedule, where the learning rate is decayed by 10 times at epoch 30, 60 and 80. The total number of epochs is still 90. As we can see, the distribution is very unstable as optimization proceeds, due to the small per-worker batch size (8 samples per worker). 
(a) and (b) show the histogram of running variances with the per-worker batch size of 8 and 128. (c) shows that when applying stable tailing strategy at the last 5 epochs the distribution of running variance in batch norm layer can approximate the one using large per-work batch size training as in (d). 
%Figure (a) and (b) are the visualization of the damp schedule, where the number of workers start with 128 (per-worker batch size is 8), and it drops to 8 (per-worker batch size is 128) at epoch 85. 
%Figure (c) is the visualization from the baseline training process, where the number of workers keeps at 8 (per-worker batch size is 128). 
%It can be seen that the distribution in Figure (c) is compactly centralized towards 0. By changing the batch size from 8 to 128, the distribution changes from Figure (a) to Figure (b), as it becomes similar to Figure (c).
}
\label{fig:bn_viz_big}
\end{figure*}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{plot/pdf/damp_spike.pdf}
  \caption{Validation curves for different GPU scheduling strategy.
  %Per-worker batch size adaption in last 10 epochs. 
  The $baseline_{128}$ and $baseline_8$ represent training with a per-GPU batch size
  of 128 or 8. 
  The {\it spike} schedule start with 8 GPUs (per-GPU batch size 128) and increase to 128 GPUs at epoch 80. 
  The {\it damp} schedule starts with 128 GPUs (per-GPU batch size 8) and reduces the number of GPU to 8 at epoch 80.}
  \label{fig:fixed_adapt}
\end{figure}

\begin{table}
\centering
\begin{adjustbox}{max width=\linewidth}

\begin{tabular}{|l|l|l|l|l|}
  \hline
  Strategy      & \# GPUs       & BS    & Schedule &  Top-1 Acc           \\ \hline
  Baseline         & 8             & 128  & / & 76.89\%             \\ \hdashline
  % Fixed         & 128           & 8     & 74.76\% ($-$2.13\%) \\
  % spike_{20,2}  & 64            & 16    & 76.37\% ($-$0.52\%) \\
  % spike_{20,2}  & 12           & 85    & 76.28\% ($-$0.61\%) \\
  Fixed total, w/o tailing     & 64          & 16   & spike$_{20, 8}$  & 76.37\% ($-$0.52\%) \\
  Fixed total, w/ tailing        & 64          & 16  & spike$_{20, 8}$   & 76.86\% ($-$0.03\%)  \\  \hdashline
  Fixed total, w/o tailing     & 128          & 8   & spike$_{20, 16}$  & 75.04\% ($-$1.85\%) \\
  Fixed total, w/ tailing        & 128          & 8  & spike$_{20, 16}$   & 76.62\% ($-$0.27\%) \\
  \hline
  \end{tabular}
\end{adjustbox}
  \centering
  \caption{Effects of using stable tailing strategy with different number of GPUs. Adapting stable tailing strategy improves the performance and nearly matches the performance using large per-GPU batch size.
  %\textbf{This table works for Adaptability Evaluations. It needs to merge results from appendix.}
  The {\it spike$_{m, n}$} denotes increasing the number of GPUs by {\it n} times at the {\it m}-th epoch.}
  \label{tab:tailing_comp}
\end{table}

%\begin{table}
%\centering
%\begin{tabular}{|c|c|c|c|}
%\hline
%    Method & Schedule & Top-1 Acc (\%) \\ \hline
%    baseline & \fixed{} &  76.68  \\
%    DPBS & \rndswitch{}(0.2, 2) & 76.49($-$0.21)  \\
%    DPBS & \rndswitch{}(0.2, 4) & 76.33($-$0.35)  \\
%    DPBS & \rndswitch{}(0.2, 8) & 76.32($-$0.36)  \\
%
%%16K &  1 & 128    & 76.27  \%  \\
%%16K &  2 & 128 \longleftrightarrow 64     & 76.21  \%  \\
%% 1K  &  8 & 128 \longleftrightarrow 16     & 76.50  \%  \\
%\hline
%
%    \caption{Validation accuracy for models trained with random switch schedule with probability $0.2$. All models are trained total batch size 8192. The random switch(5, 8) schedule randomly switches between 64 and 512 workers and achieves validation accuracy 76.32\%.}
%
%\end{tabular}
%\end{table}



% We also run $spike$ schedule at different epoch ($spike_{20, 16}$, $spike_{80, 16}$, $spike_{85, 16}$) with scale set to 16x. The result suggests that \textbf{the more epochs trained with the original per-worker batch size, the better accuracy}.

% with ratio $r$ = \{2,4,8,12,16\}, $\hat K$ = 8, and $e$ = 20. With the number of GPUs is scaled by a small factor such as $r$ = 2 and 4, the validation accuracy is almost identical to that of $base_{1024, 8}$. When the the scale ratio is large, the validation accuracy drops and is closer to that of $base_{1024, 128}$. See Table ~\ref{tab:fixed_bs_spike} for more details.

% On the other hand, in Table ~\ref{tab:fixed_bs_spike_timing} we evaluated spike schedule with $r = 16$, but at different epoch (20, 45 and 70). The final validation accuracy is all close to that of $base_{1024, 128}$.

%\begin{figure*}[tp]
%  \centering
%  \includegraphics[width=.8\textwidth]{plot/bn_viz.png}
%  \caption{Visualization of BN moving mean statistics, BN gamma parameters, BN beta parameters and Convolution parameters at stage 3, block 1 at epoch 79 and 89 for the model trained with $damp$(80, 16x) schedule.}
%  \label{fig:viz_bn}
%\end{figure*}

% \begin{figure}[tp]
%   \captionsetup[subfigure]{labelformat=empty}
%   \centering
%   \subfloat{%
%     \includegraphics[scale=0.4]{plot/spike_16x.png}
%     }%
%   \caption{Fixed total batch size, spike, r=16. The base refers to $base_{1024, 128}$.}
%   \label{fig:spike_16x}%
% \end{figure}

% \subsubsection{Other Schedule}



% \subsection{Fixing Worker Batch Size with Square Root Learning Rate Scaling}
\subsection{Fixing Worker Batch Size with LR Scaling}
\label{sec:app2-eval}

% We consider two learning rate scaling rule for adaptive learning rates: linear $F_{linear}$ and square root $F_{sqrt}$.

% \begin{equation}
% \alpha_t = F(K_t, K_0) * \alpha^*
% \end{equation}

% \begin{equation}
% F_{linear}(x, y) = \frac{x}{y}
% \end{equation}

% \begin{equation}
% F_{sqrt}(x, y) = \sqrt{\frac{x}{y}}
% \end{equation}

% \begin{figure}[bp]
%   \centering
%   \includegraphics[width=.5\textwidth]{plot/pdf/spike.pdf}
%   \caption{Validation accuracy over epochs for linear and square root scaling rule. The baseline is trained with 8 workers, while the spike schedule starts with 8 workers and increase the number of workers to 96 at epoch 20. Such a spike is very disruptive to linear scaling, while square root scaling rule leads to a milder change.}
%   \label{fig:dynamic_scale}
% \end{figure}

For fixing worker batch size, a straightforward solution is increasing the learning rate in proportion to the scale of available GPUs. 
However, we have observed the network training can be overshot and the final performance drops when increasing the number of GPUs at epoch 20 as in Table~\ref{tab:ablation}. 
Based on the analysis in the Section~\ref{sec:theory}, we hypothesize that the degraded performance is due to the large learning rate being used. 
Therefore, we explore the model accuracy as a function of the starting epochs for increasing the number of GPUs to 12 times (which refers to {\it spike schedule}) in Figure~\ref{fig:dynamic-time}. 
Comparing to the baseline method without elastic training, the network has less final accuracy loss when delaying the spike schedule, as it has relatively smaller learning rate at the changing epoch. This supports our hypothesis that the large learning rate causes degraded performance.

To stabilize the network training and achieve better accuracy, we adapt the square 
root learning rate scaling strategy. We first evaluate the network performance for
spike schedules of 12 times at different epochs in Table~\ref{tab:dynamic_spike_time} 
and find the square root scaling rule always outperforms the linear one. 
We also compare the performance for the scale factors of 8 and 16 in 
Table~\ref{tab:dynamic_spike_scale}, and the square root scaling strategy 
achieves comparable performance with 64 GPUs, and always outperforms
the linear scaling approach.



% \paragraph{Scale Evaluation}

% To better understand the performance of the linear scaling rule, we experiment spike schedules with different scales. In Table~\ref{tab:dynamic_spike_scale}, the baseline model is trained with a per-worker batch size of 128 and 8 workers. The spike schedule starts with 8 workers, and increase the number of workers to different scales at epoch 20. For both linear and square root scaling rule, a larger scale leads to worse performance. A plot of accuracy v.s. epochs with the linear scaling rule is shown in Figure~\ref{fig:collection_a_b_c}(b). As we can see, increasing the number of workers to 8 $\times$ 12 = 96 and increasing learning rate 16 times resets the network parameters such that it is almost learning from scratch again. In comparison, the square root scaling rule offers smoothness regarding changes to  learning rate, and prevents the network from ``overshooting'' when the number of workers increases.

\begin{table}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{|l|l|l|l|l|l|}
  \hline
  Strategy                  & \# GPUs   & BS   & LR & Schedule &Top-1 Acc           \\ \hline
  Baseline                  & 8         & 128  & 1x & spike$_{20, 8}$  & 76.89\%             \\ \hdashline
  Fixed worker, linear  & 64        & 128  & 8x & spike$_{20, 8}$  & 76.18\% ($-$0.71\%) \\
  Fixed worker, sqrt    & 64        & 128  & 2.83x & spike$_{20, 8}$  & 76.81\% ($-$0.08\%) \\ \hdashline
  % Linear           & 12        & 74.49\% ($-$2.40\%) \\
  % Sqrt             & 12        & \textbf{76.80}\% ($-$0.09\%) \\ \hline
  Fixed worker, linear  & 128       & 128  & 16x & spike$_{20, 16}$  & 76.09 \% ($-$0.80\%)\\
  Fixed worker, sqrt    & 128       & 128  & 4x & spike$_{20, 16}$  & 76.20\% ($-$0.69\%) \\
  \hline
  \end{tabular}
  \end{adjustbox}
  \centering
  \caption{Comparisons of linear and square root learning rate scaling strategy. 
  Top-1 validation accuracy on ImageNet is shown. 
  %The number of GPUs is increased at epoch 20 and t
  The square root learning rate scaling outperforms the linear one and
  has comparable performance with the baseline model.
  {\it spike$_{m, n}$} represents increase the number of GPUs to {\it n} times at epoch {\it m}.
  %The baseline is trained with a per-worker batch size of 128, total batch size of 1024.
  }
  \label{tab:dynamic_spike_scale}
\end{table}

% \begin{table}
% \begin{tabular}{|l|l|l|}
%   \hline
%   \# Method         & Scale     & Top-1 Acc           \\ \hline
%   Baseline          & 1        & 76.89\%             \\
%   DTBS$\sublinear$  & 8        & 76.18\% ($-$0.71\%) \\
%   DTBS$\subsqrt$    & 8        & \textbf{76.81}\% ($-$0.08\%) \\
%   % DTBS$\sublinear$  & 12       & 74.49\% ($-$2.40\%) \\
%   % DTBS$\subsqrt$    & 12       & \textbf{76.80}\% ($-$0.09\%) \\
%   DTBS$\sublinear$  & 16       & N/A \\
%   DTBS$\subsqrt$    & 16       & \textbf{76.20}\% ($-$0.69\%) \\
%   \hline
%   \end{tabular}
%   \centering
%   \caption{Validation accuracy for spike schedule at epoch 20, where the scale column indicates how much the number of workers increases at epoch 20. The baseline is trained with a per-worker batch size of 128, total batch size of 1024.
%   \textbf{Add column to include according scaled learning rate.}
%   }
%   \label{tab:dynamic_spike_scale}
% \end{table}

% \begin{table}
% \begin{tabular}{|l|l|l|}
%   \hline
%   Method            & Scale     & Top-1 Acc           \\ \hline
%   Baseline          & 1        & 76.89\%             \\
%   DPBS              & 8        & 76.37\% ($-$0.52\%) \\
%   DTBS$\sublinear$  & 8        & 76.18\% ($-$0.71\%) \\
%   DTBS$\subsqrt$    & 8        & \textbf{76.81}\% ($-$0.08\%) \\
%   % DPBS              & 12       & 76.28\% ($-$0.61\%) \\
%   % DTBS$\sublinear$  & 12       & 74.49\% ($-$2.40\%) \\
%   % DTBS$\subsqrt$    & 12       & \textbf{76.80}\% ($-$0.09\%) \\
%   DPBS              & 16       & 75.04\% ($-$0.61\%) \\
%   DTBS$\sublinear$  & 16       & $<$74.49\% ($-$2.40\%) \\
%   DTBS$\subsqrt$    & 16       & \textbf{76.20}\% ($-$0.69\%) \\
%   \hline
%   \end{tabular}
%   \centering
%   \caption{Validation accuracy for spike schedule at epoch 20, where the scale column indicates how much the number of workers increases at epoch 20. The baseline is trained with a per-worker batch size of 128, total batch size of 1024.
%   \textbf{Add column to include according scaled learning rate.}
%   }
%   \label{tab:dynamic_spike_scale}
% \end{table}

% \paragraph{Timing Evaluation}

% Given that the number of workers is spiked to a certain scale, does it matter when such change happen? In Table~\ref{tab:dynamic_spike_time} we designed the following schedules for linear scaling and square root scaling. For linear scaling, the number of workers spikes from 8 to 96, and such spike happens at different epochs (epoch 12, epoch 45, and epoch 70). For instance, spike$_{(20,12)}$ means the spike happens at epoch 12. As shown in Figure ~\ref{fig:dynamic-time}, applying the scale to later epochs is less disruptive to the optimization than earlier ones. For square root scaling, similar spike schedules are evaluated except that we are able to run with a large scale (32 times). Scaling the number of workers from 8 to 256 at epoch 20 and applying square root scaling rule worsens the validation accuracy by 1.12\%, but if the change is deferred to 25 epochs later, such a spike only results in 0.19\% loss of accuracy.

% We attribute this to both the property of the network and the effect of cosine learning rate schedule used to train the network. Recall that cosine learning rate schedule starts with a large learning rate and gradually decays the learning rate as the number of optimization steps increase. In comparison the original learning rate at epoch 45 and epoch 70 are much smaller compared to that at epoch 20, which mitigates the fact that learning rate is increased due to a large total batch size.

\begin{figure}[tp]
  \centering
  \includegraphics[width=0.9\linewidth]{plot/pdf/time.pdf}
  \caption{Comparisons of validation accuracy with different starting epochs for increasing the number of GPUs (spike schedule). 
  %over epochs for linear and square root scaling rule. 
  The baseline is trained with 8 GPUs, while the
  {\it spike\_m\_n} denotes increasing the number of GPUs by {\it n} times at {\it m} epoch.
  %while the spike schedule starts with 8 workers and increase the number of workers to 96 at epoch 20. Such a spike is very disruptive to linear scaling, while square root scaling rule leads to a milder change. 
  }
  \label{fig:dynamic-time}
\end{figure}

\begin{table}
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{|l|l|l|l|l|l|}
  \hline
          Strategy          & \# GPUs   & BS    & LR    & Schedule   & Top-1 Acc           \\ \hline
          Baseline$_{128}$  & 8         & 128   & 1x    & /         & 76.89\%             \\ \hdashline
          Fixed worker, linear            & 96        & 128   & 12x   &  spike$_{20, 12}$  & 74.49\% ($-$2.40\%) \\
          Fixed worker, sqrt              & 96        & 128   & 3.46x &  spike$_{20, 12}$  & 76.80\% ($-$0.09\%) \\ \hdashline
          Fixed worker, linear            & 96        & 128   & 12x   &  spike$_{45, 12}$  & 75.54\% ($-$1.35\%) \\
          Fixed worker, sqrt              & 96        & 128   & 3.46x &  spike$_{45, 12}$  & 76.63\% ($-$0.25\%) \\ \hdashline
          Fixed worker, linear            & 96        & 128   & 12x   &  spike$_{70, 12}$  & 76.54\% ($-$0.35\%) \\
          Fixed worker, sqrt              & 96        & 128   & 3.46x &  spike$_{70, 12}$  & 76.65\% ($-$0.23\%) \\ 
  \hline
  \end{tabular}
\end{adjustbox}
  \caption{Validation accuracy for linear scaling and square root scaling with spike schedule at different epochs. %For linear scaling rule, t
  The number of workers spikes from 8 to 96 at epoch 20, 45 and 70 respectively. %For square root scaling, the number of workers spikes from 8 to 256. 
  {\it spike$_{m, n}$} represents increase the number of GPUs to {\it n} times at epoch {\it m}.}
  \label{tab:dynamic_spike_time}
\end{table}


\begin{table*}
\begin{tabular}{|l|l|l|l|l|l|l|}
  \hline
  Strategy            & \# GPUs & BS  & LR & Schedule & Top-1 Acc      & Throughput {\tiny \it images / sec}    \\ \hline
  Baseline          & 8       & 128 & 1x &  / & 76.89\%     &   434.10\\ \hdashline
  % DPBS              & 8        & 76.37\% ($-$0.52\%) & \\
  Fixed total, w/ tailing        & 32     & 32  & 1x &  spike$_{20, 4}$ & 76.93\% ($+$0.04\%) & 683.88 (1.58x)\\
  Fixed worker, sqrt    & 32     & 128 & 2x   &  spike$_{20, 4}$ & 76.79\% ($-$0.10\%) & 1341.48 (3.09x)\\ \hdashline
  Fixed total, w/ tailing        & 64      & 16  & 1x &  spike$_{20, 8}$ & 76.86\% ($-$0.03\%) & 319.8 (0.74x)  \\
  Fixed worker, sqrt    & 64      & 128 & 2.83x &  spike$_{20, 8}$ & 76.81\% ($-$0.08\%) & 2292.88 (5.28x)\\ 
  % DPBS              & 12       & 76.28\% ($-$0.61\%) & \\
  % DTBS$\subsqrt$    & 12       & 76.80\% ($-$0.09\%) & \\ \hline
  % DPBS              & 16       & 75.04\% ($-$1.61\%) & \\
  % DPBS        & 128     & 16  & 1x & 76.54\% ($-$0.35\%) & \\
  % DTBS$\subsqrt$    & 128     & 128 & 4x   & 76.20\% ($-$0.69\%) &\\
  \hline
  \end{tabular}
  \centering
  \caption{Horizontal comparison of model accuracy and training throughput for fixed total batch size and fixed worker batch size with spike schedule at epoch 20. 
  The baseline is trained with a per-worker batch size of 128, total batch size of 1024. Throughput is measured on machines with NVidia K80 GPUs}
  \label{tab:dpbs_dtbs_comp}
\end{table*}

% \paragraph{Training Throughput}

% We benchmark the training throughput using p3.16xlarge instances on AWS. Each instance has 8 NVIDIA Volta V100 GPUs and the network bandwidth is 25 GB/s. To train ResNet-50 for 90 epochs, the baseline takes 6.5 hours. In table ~\ref{tab:throughput}, we benchmark the training thoughput with the spike(20, 4) schedule, where the number of workers increases from 8 to 32 at epoch 20. As a result, DPBS reduces training time by 22\% and DTBS reduces the training time by 55\%. In comparison, DTBS has better computation-communication ratio thanks to a large batch size is used.

% \begin{table}[h]
% \centering

% \begin{adjustbox}{width=\linewidth}

% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Method & Schedule & Avg throughput (samples/s) & Time (h) \\ \hline
% Baseline$_{128}$ & fixed & 4945 & 6.5 \\
% % fixed & 128     & 16  & 9134.66 & yyy  \\
% % fixed & 128     & 32  & 17217.72 & yyy  \\
% % fixed & 128     & 64  & 27526.08 & yyy  \\
% % fixed & 64     & 8  & 3825.87 & yyy  \\
% % fixed & 32     & 8  & 2271.88 & yyy  \\
% % fixed & 16     & 8  & 1172.53 & yyy \\
% % DPBS & spike(20, 8) & 13735 & 2.3 \\
% % DTBS & spike(20, 4) & 13735 & 2.3 \\
% DPBS & spike(20, 4) & 6260 & 5.1 \\
% DTBS & spike(20, 4) & 11100 & 2.9 \\ \hline

% \end{tabular}
% \end{adjustbox}
% \caption{Average training throughput for spike(20, 4) schedule using DPBS and DTBS methods.}
% \label{tab:throughput}
% \end{table}

\subsection{Horizontal Comparison and Dynamic Scheduling}

We have individually evaluated two different elastic training strategies, fix total batch size and fix per-worker batch size. We conduct a horizontal comparison of aforementioned approaches in the perspective of validation accuracy, training throughput with different GPU schedules, shown in Table~\ref{tab:dpbs_dtbs_comp}. 
The baseline model is trained on 8 GPUs with per-GPU batch size of 128 and achieves 76.89\% top-1 accuracy. 
For increasing the number of GPUs to 32 and 64, both fixed total batch size with stable tailing strategy and fixed worker batch size with square root scaling strategy can achieve comparable results with the baseline's.
The fixed worker batch size approach achieves better model throughput than fixed total batch size due to greater computation-communication ratio and better GPU utilization. 

% Given a computing platform with peak performance $\pi$ and memory bandwidth $\beta$, and a model with operational intensity $I$ (the ratio between the amount of work and the communication), the performance of the model $P$, measured in the number of operations performed in a unit time, can be obtained as $P \leq min(\pi, I\beta)$.
% As $I$ increases, $P$ increases until the tipping point $I = \frac{\pi}{\beta}$, after which it remains at $\pi$, thus forming a roofline shape~\citep{ofenbeck2014roof}.
% In the batch SGD setting on a GPU, because the communication comes from synchronization of parameters which is constant, while the amount of work grows linearly, both with respect to the per-GPU batch size, the performance of the model with respect to the batch size also follows the same roofline shape.
% To achieve the best throughput of GPU, our choice of the per-GPU batch size should ideally be larger the tipping point.
% When given a fixed total batch size across devices, because increasing the number of machines decreases the per-GPU batch size, even if there is more supply of spot instances it would still be more economical not to decrease the per-GPU batch size beyond the tipping point.
% Table~\ref{tab:dpbs_dtbs_comp} shows that in the fixed total setting the per-GPU batch size inevitably falls before the tipping point, and is thus not as scalable as the fixed worker setting.


In the previous sections, we mainly studied elastic training approaches with simple
GPU scheduling, a spike schedule increasing the number of GPUs at a certain epoch. 
In this section, we conduct a comprehensive benchmark of the proposed elastic
training strategies with complicated scheduling strategy 
to approximate real-word situations. 
We consider two types of random scheduling strategies as shown in Figure~\ref{fig:schedule_vis}:
1) randomly switching between two different scales of GPUs with a certain probability
({\it e.g.} {\it rand\_switch(0.2, 12x) } means randomly switch between 1x or
12x GPUs with a probability of 0.2), 
2) randomly selecting the scale of available GPUs every a few epochs
({\it e.g.} {\it rand\_step(2, 12x) } denotes that the number of available GPUs
is randomly chosen between 1x to 12x of the base GPU number).
The results are shown in Table~\ref{tab:switch_comp}, the baseline model is trained with 8 GPUs and per-GPU batch size of 128.
%Compared to the baseline, note that this time the baseline validation accuracy is slightly lower (from 76.89\% to 76.68\%) as the total batch size is increased to 8192 from 1024. 
%The three rand\_switch schedules share the value for K$_{min}$=64, and respectively set K$_{max}$=128, 256, and 512. Note that the number of workers at the last 5 epochs are all set to 64. The three models performs reasonably well and achieve 76.49\%, 76.33\%, and 76.32\% respectively.
For random GPU scheduling, both methods achieves acceptable model accuracy,
while fixed total batch size with stable tailing strategy often 
outperforms fix worker batch size with square root strategy on the validation accuracy. 
Overall, fixed total approach usually is more robust to random GPU schedule and 
has better model accuracy, while fix worker approach has better throughput.

\begin{figure}[tp]
  \centering
  \includegraphics[width=.9\linewidth]{plot/schedule_random_step.pdf}
  \caption{Visualization of two random schedules: random switch and random step. The {\it rand\_switch(0.5, 4)} schedule randomly switches between 1x and 4x number of GPUs. The {\it rand\_step(5, 4)} schedule randomly changes the number of GPUs between 1x and 4x for every 5 epochs. }
  \label{fig:schedule_vis}
  \vspace{-3em}
\end{figure}

% \begin{figure}[tp]
% \centering
% \subfigure[rand\_switch(0.5, 4)]{
% \includegraphics[width=.35\textwidth]{plot/schedule_random_switch_1.pdf}
% }\hspace{}
% \subfigure[rand\_step(5, 4)]{
% \includegraphics[width=.35\textwidth]{plot/schedule_random_switch_2.pdf}
% }
% \caption{ Visualization of two random schedules: random switch and random step. }
% \label{fig:schedule_vis}
% \end{figure}

%Under the same scale schedule, we compare the accuracy and throughput for DPBS and DTBS in Table~\ref{tab:dpbs_dtbs_comp}. 

%\subsubsection{Accuracy and throughput}

%\subsubsection{Robustness}

%Finally we evaluate and compare the effect of multiple random changes in two schedules.

% \paragraph{Random Switch Schedules}

% This schedule is generated as follows: at the beginning of each epoch, the number of workers switches between two numbers (K$_{min}$ and K$_{max}$) with a probability.


\begin{table*}
\begin{tabular}{|l|l|l|l|l|l|} 
  \hline
    Strategy & Range of \# GPUs & Range of BS & Range of LR & Schedule & Top-1 Acc (\%) \\ \hline
    baseline & 8 & 128 & 1x & \fixed{} &  76.89\%  \\ \hdashline
    %DPBS & 16 & 64 & 1x & \rndswitch{}(0.2, 2) & 76.49\%($-$0.21\%)  \\
    %DTBS$\subsqrt$ & 16 & 128 & 1.414x  & \rndswitch{}(0.2, 2) & N/A  \\ \hline
    %DPBS & 32 & 32 & 1x & \rndswitch{}(0.2, 4) & 76.33\%($-$0.35\%)  \\
    %DTBS$\subsqrt$ & 32 & 128 & 2x & \rndswitch{}(0.2, 4) & N/A  \\ \hline
    %DPBS & 64 & 16 & 1x & \rndswitch{}(0.2, 8) & 76.32\%($-$0.36\%)  \\
    %DTBS$\subsqrt$ & 64 & 128 & 2.828x & \rndswitch{}(0.2, 8) & N/A  \\ \hline
    Fixed total, w/ tailing & 8 $\leftrightarrow$ 96 & 128 $\leftrightarrow$ 10 & 1x & \rndswitch{}(0.2, 12x) & 76.72\%($-$0.17\%)  \\
    Fixed worker, sqrt & 8 $\leftrightarrow$ 96 & 128 & 1x $\leftrightarrow$ 3.46x & \rndswitch{}(0.2, 12x) & 76.18\%($-$0.71\%) \\ \hdashline
    Fixed total, w/ tailing & 8 $\leftrightarrow$ 128 & 128 $\leftrightarrow$ 8 & 1x & \rndstep{}(2, 16x) & 76.88\%($-$0.01\%) \\
    %DPBS & N/A & N/A & 1x & \rndstep{}(N/A, N/A) & N/A  \\
    %DPBS & N/A & N/A & 1x & \rndstep{}(N/A, N/A) & N/A  \\
    Fixed worker, sqrt & 8 $\leftrightarrow$ 128 & 128 & 1x $\leftrightarrow$ 2.83x & \rndstep{}(2, 16x) & 76.59\%($-$0.30\%)  \\
  \hline
  \end{tabular}
  \centering
  \caption{Horizontal comparison of model accuracy with random schedules. 
  The {\it rand\_switch(0.2, 12x)} schedule randomly switches between 1x and 12x number of GPUs. The  {\it rand\_step} (2, 16x) schedule randomly changes the number of GPUs between 1x and 16x for every 2 epochs.}
  \label{tab:switch_comp}
\end{table*}

% \paragraph{Random Step Schedules}

% In this schedule, we change the number of GPUs to a random number between 8 and 128 every 5 epochs, which simulates an unstable training environment.


% \begin{table*}
% \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%     Method & Max \# GPUs & Min BS & Max LR & Schedule & Top-1 Acc (\%) \\ \hline
%     baseline-1024-128 & 8 & 128 & 1x & \fixed{} &  76.89\%  \\
%     DPBS & 128 & 8 & 1x & \rndstep{}(2, 16x) & 76.88\% \\
%     %DPBS & N/A & N/A & 1x & \rndstep{}(2, 16x) & 77.14\%  \\
%     %DPBS & N/A & N/A & 1x & \rndstep{}(2, 16x) & 76.80\%  \\
%     DTBS$\subsqrt$ & 128 & 128 & 2.828x & \rndstep{}(2, 16x) & 76.59\%  \\

%     %DTBS$\subsqrt$ & N/A & 128 & N/A & \rndstep{}(2, 16x) seed 3 & 76.16  \\
%     %DTBS$\subsqrt$ & N/A & 128 & N/A & \rndstep{}(2, 16x) seed 2 & 76.57  \\
%   \hline
%   \end{tabular}
%   \centering
%   \caption{Validation accuracy for models trained with random switch schedule with probability $0.2$. All models are trained total batch size 102. The random switch(5, 8) schedule randomly switches between 64 and 512 workers and achieves validation accuracy 76.32\%.}
%   \label{tab:step_comp}
% \end{table*}

\begin{table*}
\begin{tabular}{l|l|l|l|l}
    \hline
     Method & Max \# GPUs & ResNet-50 & MobileNet 1.0 & Inception V3 \\ \hline\hline
     Baseline & 1 & 76.89 & 72.16 & 77.78 \\ \hline
     Baseline & 12 & 76.72 & 72.02 & 77.02 \\ \hdashline
     Linear  & 12 & 76.78 ($\pm$ 0.59) & 72.12 & 77.72 \\ \hdashline
     Linear Warmup & 12 & 77.00 ($\pm$ 0.29) & 72.27 & 77.89 \\ \hline
     Baseline & 16 & 76.08 & &  \\ \hdashline
     Linear & 16 & 76.14 & 71.56 ($\pm$ 0.26) & 76.88 \\ \hdashline
     Linear Warmup & 16 & 76.73 ($\pm$ 0.73) & 71.99 & 77.61 \\ \hline
\end{tabular}
\centering
\caption{Validation accuracy for three models trained with random steps.}
\label{tab:rand_step_cls}
\end{table*}


% \begin{figure}[tp]
%  \centering
%  \includegraphics[width=.5\textwidth]{plot/pdf/random_step_fixed.pdf}
%  \caption{Validation accuracy for rand step(5, 16x) schedule for DPBS.}
%  \label{fig:fixed-rand-step}
% \end{figure}

%Figure~\ref{fig:fixed-rand-step} shows the result for \rndstep{}(5, 16) using DPBS.
%The number of workers is changed to a random number between 8 and 128 every 5 epochs.
%DPBS achieves 76.8\% validation accuracy, which is 0.09\% worse in accuracy compared to the baseline model.

%We also extend experiments with multiple changes during training including with random step and random switch schedules. Figure~\ref{fig:step-dynamic} shows the result for \rndstep{}(5, 16) using linear and square root scaling rules. The number of workers is changed to a random number between 8 and 128 every 5 epochs. Square root scaling reaches validation accuracy of 76.60\% (0.29\% loss of accuracy), while linear scaling performs much worse. In Figure~\ref{fig:random_switch_acc}, we use \rndswitch{} schedule which alternates between 8 and 96 workers with probability 0.25 at the beginning of each epoch, and square root scaling rule achieves 76.14\% validation accuracy.


% \begin{table}[!htb]
%     \begin{minipage}{.5\linewidth}
%       \centering
%         \begin{tabular}{|c|c|c|c|}
%         \hline
%         Rule & Schedule & B & Top-1 Acc \\ \hline
%         &\fixed{}& 1024  & 76.89\%  \\
%         &\fixed{}& 12288  & 76.27\%  \\
%         &\fixed{}& 16384  & 76.18\%  \\
%         linear &8x  & 1024 $\rightarrow$ 8192   & 76.18\%  \\
%         linear &12x  & 1024 $\rightarrow$ 12288   & 74.49\%  \\
%         sqrt& 8x  & 1024 $\rightarrow$ 8192     & 76.81\%  \\
%         sqrt& 12x & 1024 $\rightarrow$ 12288   & 76.80\%  \\
%         sqrt& 16x & 1024 $\rightarrow$ 16384   & 76.20\%  \\
%         linear &12x at epoch 20  & 1024 $\rightarrow$ 12288   & 74.49\%  \\
%         linear &12x at epoch 45  & 1024 $\rightarrow$ 12288   & 75.54\%  \\
%         \hline
%         \end{tabular}
%         \centering
%         \parbox{6cm}{
%             \newline
%             \caption{Validation accuracy with $spike$ schedule at epoch 20. The mini-batch size per worker ($S$) for all experiments is set to 128. \label{tab:adaptive_spike_scale}}
%         }
%     \end{minipage}%
%     % \begin{minipage}{.5\linewidth}
%     %   \centering
%     %     \begin{tabular}{|l|c|c|c|c|}
%     %     \hline
%     %     Schedule & Total Batch Size & Top-1 Acc \\ \hline
%     %     \fixed{}     & 1024  & 76.89\%  \\
%     %     \fixed{}     & 12288  & 76.27\%  \\
%     %     linear 12x at epoch 20  & 1024 $\rightarrow$ 12288   & 74.49\%  \\
%     %     linear 12x at epoch 45  & 1024 $\rightarrow$ 12288   & 75.54\%  \\
%     %     \hline
%     %     \end{tabular}
%     %     \newline
%     %     \centering
%     %     \parbox{8.2cm}{
%     %         \caption{Validation accuracy with spike schedule at epoch 20. The mini-batch size per worker ($S$) for all experiments is set to 128. \label{tab:adaptive_spike_time}}
%     %     }
%     % \end{minipage}
% \end{table}


% However, we did not observe loss of accuracy with sqrt scaling rule in Figure~\ref{fig:time_sqrt}.

% TODO time sensitive : sqrt needs a better upper bound.

% \begin{figure}[H]
% \centering
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.2]{plot/adaptive_scale.png}
%   \caption{Spike schedule, e = 20. "linear\_8x" means linear scaling rule, K increased by 8x. "sqrt\_12x" means square root scaling rule, K increased by 12x.}
%   \label{fig:adaptive_scale}
% \end{minipage}%
% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.2]{plot/0_2_switch_12x.png}
%   \caption{Random Switch GPU schedule, sqrt learning rate scaling, p = 0.2, r = 12}
%   \label{fig:switch_12x}
% \end{minipage}%

% \begin{minipage}{.5\textwidth}
%   \centering
%   \includegraphics[scale=0.2]{plot/adaptive_spike_12x.png}
%   \caption{Spike schedule with linear scaling rule. r = 12. e = 20, 45, 70 respectively.}
%   \label{fig:adaptive_spike_12x}
% \end{minipage}
% \end{figure}

% Optional section
% \subsubsection{Random Schedule}

% In Figure~\ref{fig:random}, we experimented with adaptive learning rate with linear and square root scaling rule with random GPU schedule. The result shows that both scaling rule works well if the number of GPUs is increased to up to 5x.

% Optional figure
% \begin{figure}[tp]
%   \captionsetup[subfigure]{labelformat=empty}
%   \centering
%   \subfloat{%
%     \includegraphics[scale=0.25]{plot/adaptive-linear-sqrt-8x.pdf}
%     }%
%   \caption{Random GPU schedule, r = 8.}
%   \label{fig:random}
% \end{figure}

% \begin{figure}[tp]
%   \centering
%   \includegraphics[width=.5\textwidth]{plot/pdf/random_switch.pdf}
%   \caption{Validation accuracy for random switch schedule. The baseline model uses per worker batch size 128 and total batch size 1024.}
%   \label{fig:random_switch_acc}
% \end{figure}

\subsection{Elastic Training for Object Detection}

We go beyond the image classification problem to study the elastic training 
on object detection task. 
The fixed worker batch size approach is used in this experiment, 
as large throughput is highly desirable.
We train Single Shot Multi-box Object Detector (SSD) \cite{liu2016ssd} with input image 
size $512 \times 512$ on MS-COCO dataset~\cite{lin2014microsoft}  with ResNet-50 backbone. 
%SSD network extends backbone network with multiple convolutional branches connected to different downsampling layers in order to gather detection results from various receptive fields. 
We follow the experimental settings in Liu \textit{et.al.} \cite{liu2016ssd}, which implements extensive data augmentation, hard negative sampling mining, and loss normalization by valid object count. The author used learning rate of $0.001$ and batch-size 32 for training.
The baseline model is trained with $0.008$ and batch size 256 on 32 GPUs, with a cosine learning rate schedule. %For SSD we omit the validation result with DPBS, since the accuracy will exactly match the baseline.
{\it random\_step(5, 9x)} scheduling indicates that the number of GPUs is updated every
5 epochs with a range of 9 times of the base number of GPUs. 
We evaluate fixed worker batch size approach with both linear and square root 
learning rate scaling strategies as shown in Table~\ref{tab:ssd}. 
The SSD training diverges with linear scaling strategy due to large learning rate 
causing network overshoot.
For square root scaling, the model can achieve acceptable results with less than 1.5\% 
mAP loss for both 288 and 512 number of GPUs.

\begin{table*}[h]
\begin{center}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Strategy         & \# GPUs & BS &  LR & Schedule & mAP \\ \hline
Baseline         & 32  & 8  & 1x & / & 28.6  \\ \hdashline
Fixed worker, linear  & 288 & 8 & 9x & rand\_step(5, 9x) & diverged   \\
Fixed worker, sqrt    & 288  & 8 & 3x & rand\_step(5, 9x)  & 27.5   \\ \hdashline
Fixed worker, linear  & 512 & 8 & 16x & rand\_step(5, 16x)  & diverged   \\
Fixed worker, sqrt    & 512 & 8 & 4x & rand\_step(5, 16x)  & 27.1   \\ \hline

\end{tabular}
\end{adjustbox}
\end{center}
\caption{SSD validation mean average precision on MS COCO 2017 val set. The  {\it random\_step} (5, 9x) schedule randomly changes the number of GPUs between 1x and 9x for every 5 epochs.}
\label{tab:ssd}
\end{table*}



